The Fast Johnson-Lindenstrauss Transform is Even Faster

The seminal Fast Johnson-Lindenstrauss (Fast JL) transform by Ailon and Chazelle (SICOMP'09) embeds a set of $n$ points in $d$-dimensional Euclidean space into optimal $k=O(\varepsilon^{-2} \ln n)$ dimensions, while preserving all pairwise distances to within a factor $(1 \pm \varepsilon)$. The Fast JL transform supports computing the embedding of a data point in $O(d \ln d +k \ln^2 n)$ time, where the $d \ln d$ term comes from multiplication with a $d \times d$ Hadamard matrix and the $k \ln^2 n$ term comes from multiplication with a sparse $k \times d$ matrix. Despite the Fast JL transform being more than a decade old, it is one of the fastest dimensionality reduction techniques for many tradeoffs between $\varepsilon, d$ and $n$. In this work, we give a surprising new analysis of the Fast JL transform, showing that the $k \ln^2 n$ term in the embedding time can be improved to $(k \ln^2 n)/\alpha$ for an $\alpha = \Omega(\min\{\varepsilon^{-1}\ln(1/\varepsilon), \ln n\})$. The improvement follows by using an even sparser matrix. We also complement our improved analysis with a lower bound showing that our new analysis is in fact tight.

==> BackupUpper.tex <==
\section{Upper Bound}
In this section we give the prove of \Cref{phdtheoremuppermain}. We start by giving the high level ideas of our proof. As in previous works, our analysis follows by arguing that for any fixed unit vector $x$, it holds with probability at least $1-\delta$ that $\|k^{-1/2}PHDx\| \in (1 \pm \eps)$. To preserve the pairwise distance between any pair of points in a set $X$ of $n$ points (guarantee~\eqref{eq:jl}), we now set $\delta = 1/n^3$ and do a union bound over all normalized pairwise difference vectors $z/\|z\|$ for $z=x-y$ with $x,y\in X$. Thus from here on, we focus on preserving the norm of a single unit vector with probability $1-1/n^3$.

First, we observe that $HD$ is a unitary matrix and thus $\|HDx\|=\|x\|=1$ for a unit vector $x$. Moreover, any single coordinate $(HDx)_i$ equals $d^{-1/2} \sum_{j=1}^d \sigma_j x_j$, where the $\sigma_j = D_{j,j}\sign(H_{i,j})$'s are independent Rademacher random variables. Thus in line with the analysis by Ailon and Chazelle~\cite{Ailon2009TheFJ}, we get that any coordinate $(HDx)_i$ is bounded by $O(\sqrt{\ln(n)/d})$ in absolute value with probability $1-1/n^5$. A union bound over all $d \leq n$ coordinates (this assumption is also made in previous work) gives that all coordinates of $HDx$ are bounded by $O(\sqrt{\ln(n)/d})$ with probability $1-1/n^4$.

Up to this point, our analysis has followed that by Ailon and Chazelle uneventfully. What remains now is to argue that $k^{-1/2}\|Pu\| \in (1 \pm \eps)$ with high probability when $u = HDx$ is a unit vector with all coordinates bounded by $O(\sqrt{\ln(n)/d})$. This is where our analysis departs from previous work.

To simplify the analysis, we will argue that $k^{-1}\|Pu\|^2 \in (1 \pm \eps)$ with probability $1-1/n$. Taking square roots on both sides and adjusting $\eps$ by a constant factor implies $k^{-1/2} \|Pu\| \in (1 \pm \eps)$. To understand the distribution of $\|Pu\|^2$ for a fixed $u$, notice that the $i$'th coordinate of $Pu$ is given by $\sum_{j=1}^d q^{-1/2} u_j b_{i,j} N_{i,j}$ by definition of $P$. Let us assume that the Bernoulli random variables $b_{i,j}$ have been fixed. In this case, $(Pu)_i$ is a sum of weighted and independent $\Norm(0,1)$ random variables. Hence $(Pu)_i$ is itself $\Norm(0,q^{-1} \sum_{j=1}^d b_j u_j^2)$ distributed. Now define $Z_i = \sum_{j=1}^d b_j u_j^2$ and let $N_1,\dots,N_k$ be independent $\Norm(0,1)$ random variables. We see that, for fixed values of all Bernoullis, $\|Pu\|^2$ is distributed as $\sum_{i=1}^k q^{-1} (\sqrt{Z_i} N_i)^2$, which is equal in distribution to $\sum_{i=1}^k q^{-1} Z_i N_i^2$. Our proof now has two steps: 1.) Give a bound on the $Z_i$'s that hold with high probability over the random choice of the Bernoullis $b_{i,j}$, and 2.), use the bound on the $Z_i$'s to argue that $\sum_{i=1}^k q^{-1} Z_i N_i^2$ behaves in a desirable manner.

In order to understand what type of bounds we need on the $Z_i$'s, we start by examining step 2. For this step, we need a tail bound on $\sum_{i=1}^k q^{-1} Z_i N_i^2$. When the $Z_i$'s are fixed, this is a weighted sum of sub-exponential random variables. To analyse it, we use Proposition 3 from \cite{zhang2020nonasymptotic}, which gives upper bounds on the tails of sub-exponential random variables:

\begin{proposition}[\cite{zhang2020nonasymptotic}]\label{chisquareuppertails1} Let $Y_{1}, \ldots, Y_{k}$ be independent centred sub-exponential random variables in the sense that $\mathbb{E} \exp \left(t Y_{i}\right) \leq \exp \left(C t^{2}\right)$ for all $|t| \leq c'$. Then for every $a_{1}, \ldots, a_{k}\in \mathbb{R}$ and  $R= a_{1} Y_{1}+\cdots+a_{k} Y_{k}$ satisfies
$$
\begin{array}{ll}
\mathbb{P}(|R| \geq x) \leq 2 \exp \left(-\frac{c x^{2}}{\|a\|_{2}^{2}}\right), & \forall 0 \leq x \leq \frac{\|a\|_{2}^{2}}{\|a\|_{\infty}} \\
\mathbb{P}(|R| \geq x) \leq 2 \exp \left(-\frac{c x}{\|a\|_{\infty}}\right), & \forall x \geq \frac{\|a\|_{2}^{2}}{\|a\|_{\infty}}
\end{array}
$$
\end{proposition}
Note that for a standard normal distribution $N$, we have that the square of the normal distribution centred (i.e. $N^2-1$) is a sub-exponential random variable in the spirit of \Cref{chisquareuppertails1}. This can be seen by $|t|\leq 0.3$ we have that
\begin{gather*}
\E\left[ \exp\left(t(N^2-1) \right)\right] \leq \E\left [\exp(tN^2)\right ]=(1-2t)^{-\frac{1}{2}}=\exp\left(-\frac{\ln(1-2t)}{2}\right)\leq \exp\left(\frac{(-2t)+(-2t)^2}{2}\right)\leq \exp(2t^2)
\end{gather*}
where the first equality follows by the $\chi^2$-distributions moment generating function and the second to last inequality follows by $-\ln(1+x)\leq x+x^2$ for $x>-0.68$. Thus we can apply \Cref{chisquareuppertails1} to $\sum_{i=1}^k q^{-1} Z_i N_i^2$ by rewriting as $\sum_{i=1}^k q^{-1} Z_i (N_i^2-1) + \sum_{i=1}^k q^{-1} Z_i$. The latter term is constant when the Bernouillis have been fixed and thus we may use \Cref{chisquareuppertails1}.

Examining \Cref{chisquareuppertails1}, we see that we need two bounds on the $Z_i$'s, one on $\sum_i Z_i^2$ and one on $\max_i |Z_i|$. Thus for step 1., we focus on giving bounds on these two quantities. For this, we will use that $u = HDx$ has all coordinates bounded in absolute value as observed earlier. For bounding $\max_i Z_i$, we prove the following lemma:

\begin{lemma}\label{ublemma1}
For $i=1\ldots,k$ let $Z_i=\sum_{j=1}^d u_j^2 b_{i,j}$ where the $b_{i,j}$'s are independent Bernoulli random variables with success probability $q$ and the $u_j^2$'s positive real numbers bounded by $1/m$ and summing to 1. We then have for $\varepsilon\leq 1/4$ that
\begin{gather*}
\ppp(\max_{i=1,\ldots,k} Z_i>\frac{q}{2\varepsilon })\leq k\exp\left(-\frac{mq\ln(1/\varepsilon)}{32\varepsilon}\right).
\end{gather*}
\end{lemma}

Next, we also need a bound on $\sum_i Z_i^2$ as noted earlier. For this, we prove the following lemma:

  \begin{lemma}\label{ublemma3}
    Let $Z_1,\dots,Z_k$ be i.i.d. random variables distributed as the $Z_i$'s in \Cref{ublemma1} and assume that $\log_2(k)$ is an integer. Then for any $t \geq 64\cdot24 e^3 q^2 k$ and $q \geq 8/(em)$, we have:
    \[
      \Pr[\sum_{i=1}^k Z_i^2 >  t] < 6\exp\left(-\frac{m\sqrt{t}\ln(\sqrt{t/2^{3}}/(eq))}{44\cdot2^{\frac{5}{2}}} \right)
      \]
  \end{lemma}

Unfortunately, \Cref{ublemma3} does not capture all tradeoffs between $\eps, d$ and $n$ that we need. Thus we also need the following alternative to \Cref{ublemma3}:

 \begin{lemma}\label{ublemma4}
 Let $Z_1,\dots,Z_k$ be i.i.d. random variables distributed as the $Z_i$'s in \cref{ublemma1}, with the embedding dimension $k$ being $ \cubiii\ln( 1/\delta)/\varepsilon^2$ where $\cubii\geq 1$ and such that $\log_2 k$ is an integer, $q =\cubii \varepsilon$ and $m=\cubiiii d/\ln \delta$, where $\cubiiii\geq1$ and such that $m$ is an integer. For $\varepsilon$ sufficiently small and $t= \cubi \ln(1/\delta)$, where $\cubi$ is such that $\cubi /(2\cubii^3)\geq e^8$ and $\log_2 t$ is an integer, we then have that 
    \[
      \Pr[\sum_{i=1}^k Z_i^2 >  t] \leq \frac{\exp\left (-\frac{tm\ln(1/q)}{400\sqrt{2}}\right )}{1-\exp\left (-\frac{tm\ln (1/q)}{400\sqrt{2}}\right )}.
    \]
  \end{lemma}

With the central lemmas laid out, we now give the full proof details by following the above proof outline. The proofs of \Cref{ublemma1}, \Cref{ublemma3} and \Cref{ublemma4} can be found in the appendix.

\paragraph{Proof of \Cref{phdtheoremuppermain}.}
\begin{proof}
Let the embedding dimension $k$ be $\cubiii\ln (1/\delta)/\varepsilon^2$, such that $k$ is a power of 2 and $\cubiii\geq32$ is a constant. Let further $m=\cubiiii d/\ln (1/\delta)$, where $\cubiiii\geq 1$ is a constant and such that $m$ is an integer. Let the success probabilities of the binomial random variables $b_{i,j}$ in $P$ be 
\[
q=\max(\cubiiiii/m,\cubii\varepsilon\min\left (1,\ln (k/\delta)/(m\ln (1/\varepsilon))\right )).
\]
 Assume for now that $u$ is a vector in $\mathbb{R}^d$ such that $u_i^2\leq 1/m$ for all $i=1,\ldots,d$ and $\norm{u}=1$. Now using the construction of $P$ and the rules of linear combinations of independent standard normal distributions have that 
\begin{gather*}
\norm{Pu}\stackrel{}{=}\sum_{i=1}^k \left(\sum_{j=1}^{d} \sqrt{1/q}u_j b_{ij} N_{ij}\right)^2\stackrel{d}{=}\sum_{i=1}^\clbiiiii \frac{1}{q}Z_i  N_{i}^2
\end{gather*}
where the $Z_i$'s are equal to $\sum_{j=1}^{d}  u_j^2b_{ij}$ and the $N_i$'s are independent standard normal random variables. Hence we conclude that the norm squared of $Pu$ is distributed as a weighted sum of $\chi^2$ variables, with random weights, and we will in the following work with this random variable.

We first prove a bound on $\sum_i Z_i$. For this, notice that $\sum_{i=1}^k Z_i$ is a sum of independent random variables, where the $Z_i$'s are themselves sums of independent random variables with values between $[0,1/m]$. Furthermore, we have $\E\left[Z_i\right]=q$, implying that $\E [\sum_{i=1}^k mZ_i]=qmk$. We therefore get by a Chernoff bound that 
\begin{gather*}
\ppp(\sum_{i=1}^k Z_i\not\in (1\pm\varepsilon)qk)=\ppp(\sum_{i=1}^k mZ_i\not\in (1\pm\varepsilon)qmk)\leq 2\exp\left(-\frac{qmk\varepsilon^2}{3}\right)\leq 2\delta^{\cubiii^2 /3},
\end{gather*}
where the last inequality follows by $q\geq \cubiiiii/m$ and $k=\cubiiiii \ln(1/\delta)/\eps^2$, so $qmk\varepsilon^2\geq\cubii^2\ln( 1/\delta)$. Thus we have $\sum_{i=1}^k Z_i\in (1\pm\varepsilon)qk$ with probability at least $1-2\delta^{\cubiii^2/3}$.

We now do a case analysis based on the value of $q$. Our goal is to show that $\|Pu\|^2 = \sum_i Z_i N_i^2/q \in (1 \pm \eps)k$ with high probability (conditioned on $u$ having bounded coordinates as remarked earlier).

\subsubsection*{Cases $q=\cubiiiii/m$ and $q= \cubii\varepsilon\ln(k/\delta)/(m\ln(1/\varepsilon))$}
We treat the cases $q=\cubiiiii/m$ and $q= \cubii\varepsilon\ln(k/\delta)/(m\ln(1/\varepsilon))$ in a similar manner.

In both these cases, we have $q\geq  \cubii\varepsilon\ln(k/\delta)/(m\ln(1/\varepsilon))$ (due to the $\max$ in the definition of $q$). Hence \Cref{ublemma1} implies that $\|Z\|_\infty=\max_{i=1,\ldots,k} Z_i \leq q/(2\varepsilon) $ with probability at least $1-k\exp(-(mq\ln(1/\varepsilon))/(32\varepsilon))\geq 1-\delta^{\cubii/32}$ (which follows by $mq\ln (1/\varepsilon)/\varepsilon\geq \cubii \ln(k/\delta)$). 

At the same time, since we in these cases have that $q\geq \cubii\varepsilon\ln(k/\delta)/(m\ln(1/\varepsilon))$ (by the $\max$ in the definition of $q$), \Cref{ublemma3} yields that $\|Z\|^2=\sum_{i=1}^k Z_i^2\leq 64\cdot24 \cdot e^3q^2k$ with probability at least  


\begin{gather*}1-6\exp\left(-\frac{m\sqrt{64\cdot24 \cdot e^3q^2k}\ln(\sqrt{(64\cdot24 \cdot e^3q^2k)/(2^{3})}/(eq))}{44\cdot2^{\frac{5}{2}}} \right)\\
\geq 1- 6\exp\left(-\frac{3\cubii\ln \left(\frac{k}{\delta}\right)\sqrt{\ln\left(1/\delta\right) }\ln\left(22\sqrt{k}\right)}{\ln\left(1/\eps \right) } \right)\\
\geq 1-6\left(\frac{\delta}{k}\right)^{3\cubii}\geq 1-6\delta^{3\cubii}
\end{gather*}
where we in the first inequality used that $(\sqrt{64\cdot24e^3})/(44\cdot 2^{2/5})\geq 3$, $\sqrt{(64\cdot24e^3)/2^3}\geq 22$ and $mq\sqrt{k}\geq
 (c_1\varepsilon\ln(k/\delta)/\ln(1/\varepsilon))\sqrt{c_1\ln (1/\delta)/\varepsilon^2}
 =(\cubii \ln \left(k/\delta\right)\sqrt{\ln(1/\delta) })/(\ln\left(1/\eps \right))$ and in the second inequality that $\ln (22\sqrt{k})/(\ln\left(1/\eps\right))=\ln(22\sqrt{c_1\ln\left(1/\delta\right)/\varepsilon^2})/(\ln\left(1/\eps \right))\geq 1$.

 Hence in these cases we have that $\sum_{i=1}^k Z_i\in (1\pm\varepsilon)qk$, $\|Z\|_\infty=\max_{i=1,\ldots,k} Z_i \leq \frac{q}{2\varepsilon} $ and $\|Z\|^2=\sum_{i=1}^k Z_i^2\leq 64\cdot 24 e^3q^2k$ with probability at least $1-9\delta^{\cubiii/32}$. We call such outcomes of the $Z_i$'s \emph{desirable}.
 
 We now notice that for desirable outcomes of the $Z_i$'s, we have from \Cref{chisquareuppertails1} that if $\varepsilon \sum_{i=1}^k Z_i \geq \|Z\|^2/\|Z\|_\infty$, then (with probability over the $N_i$'s)
\begin{gather*}
\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\not\in (1\pm\varepsilon)\sum_{i=1}^k \frac{1}{q}Z_i\right)\leq 2\exp\left(-\frac{c\varepsilon\sum_{i=1}^k Z_i}{\|Z\|_\infty}\right)\leq 2\exp\left(-\frac{c\varepsilon qk/2}{q/(2\varepsilon) }\right)= 2\delta^{c \cubiii},
\end{gather*}
where we in the equality have used that $k=\cubiii \eps^{-2} \ln(1/\delta)$. On the other hand, if $\varepsilon \sum_{i=1}^k Z_i \leq \|Z\|^2/\|Z\|_\infty$, then by \Cref{chisquareuppertails1}:
\begin{gather*}
\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\not\in (1\pm\varepsilon)\sum_{i=1}^k \frac{1}{q}Z_i\right)\leq 2\exp\left(-\frac{c(\varepsilon\sum_{i=1}^k Z_i)^2}{||Z||^2}\right)\leq 2\exp\left(-\frac{c\varepsilon^2q^2k^2}{64\cdot96e^3q^2k}\right)= 2\delta^{c \cubiii/(64\cdot 96 e^3)}.
\end{gather*}
By this we conclude that for desirable outcomes of the $Z_i$'s, if we define the constant $r_1=c/(64\cdot 96 e^3)$, then we have (with probability over the $N_i$'s):
\begin{gather*}
1-2\delta^{r_1 \cubiii} \leq\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\in (1\pm\varepsilon)\sum_{i=1}^k \frac{1}{q}Z_i)\right)\leq\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\in (1\pm4\varepsilon)k\right) 
\end{gather*}
where we in the last inequality have used that for the desirable outcomes of the $Z_i$'s, we have $\sum_{i=1}^k Z_i\in (1\pm\varepsilon)qk$.

Since the $Z_i$'s and the $N_i$'s are independent, it follow from the above that with probability at least $(1-2\delta^{r_1\cubiii})\cdot(1-9\delta^{\cubii/32})\geq1-11\delta^{\min(r_1,1/32)\cubiii}$ we have $\sum_{i=1}^k N_i^2Z_i/q\in (1\pm4\varepsilon)k$.

\subsubsection*{Case $q=\cubii\varepsilon$}
In the case that $q=\cubii\varepsilon$ (we assume that $\varepsilon$ is less than $\cubii/2$), it follows from \Cref{ublemma4}  with $\cubi\geq 2\cubii^3e^8$ that $\|Z\|^2=\sum_{i=1}^k Z_i^2\leq 2\cubii^3e^8 \ln\left(1/\delta\right)$ with probability at least  
\begin{gather*}
1-\frac{\exp\left (-\frac{2\cubii^3e^8 \ln\left(1/\delta\right)m\ln (1/q)}{400\sqrt{2}}\right)}{1-\exp\left (-\frac{2\cubii^3e^8 \ln\left(1/\delta\right)m\ln (1/q)}{400\sqrt{2}}\right )}\\
\geq 1-\frac{\delta^{7\cubiiiii}}{1-\delta^{7\cubiiiii}}
\\
\geq 1-2\delta^{7\cubiiiii},
\end{gather*}
where we in the second inequality have used that so $2\cubii^3e^8\ln (1/q)/(400\sqrt{2})\geq32^3e^8 \ln (2)/(200\sqrt{2})\geq 7$.

Thus we conclude that with probability at least $1-4\delta^{\frac{\cubii}{3}}$ we have $\sum_{i=1}^k Z_i\in (1\pm\varepsilon)qk$ and $\|Z\|^2=\sum_{i=1}^k Z_i^2\leq 2\cubii^3e^8 \ln\left(1/\delta\right)$. In this part of the case analysis, we refer to such outcomes as \emph{desirable}.

Now for desirable outcomes of the $Z_i$'s, we get again using \Cref{chisquareuppertails1} that if $\varepsilon \sum_{i=1}^k Z_i \geq \|Z\|^2/\|Z\|_\infty$, then with probability over the $N_i$'s, and using the trivial bound that the $Z_i$'s are no more than 1, it follows that
\begin{gather*}
\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\not\in (1\pm\varepsilon)\sum_{i=1}^k \frac{1}{q}Z_i\right)\leq 2\exp\left(-\frac{c\varepsilon\sum_{i=1}^k Z_i}{\|Z\|_\infty}\right)\leq 2\exp\left(-\frac{c\varepsilon qk}{2}\right)= 2\delta^{\frac{c \cubiii^2}{2}},
\end{gather*}
where the equality follows from $\varepsilon qk=c_1^2\ln\left(1/\delta\right)$. If instead $\varepsilon \sum_{i=1}^k Z_i \leq \|Z\|^2/\|Z\|_\infty$, \Cref{chisquareuppertails1} yields:
\begin{gather*}
\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\not\in (1\pm\varepsilon)\sum_{i=1}^k \frac{1}{q}Z_i\right)\leq 2\exp\left(-\frac{c(\varepsilon\sum_{i=1}^k Z_i)^2}{\|Z\|^2}\right)\leq 2\exp\left(-\frac{c\varepsilon^2q^2k^2}{2\cubii^3e^8\ln\left(1/\delta\right)}\right)\leq 2\delta^{c \cubiii/(2e^8)}.
\end{gather*}
Where the last inequality follows from $\varepsilon^2q^2k^2/(\ln(1/\delta))=\cubii^4\varepsilon^4\ln^2(1/(\delta) /(\varepsilon^4\ln\left(1/\delta\right))\geq \cubii^4\ln\left(1/\delta\right)$.

Now define the constant $r_2=c/(2e^8)$. From the above, we conclude that for desirable outcomes of the $Z_i$'s, we have with probability (over the $N_i$'s):
\begin{gather*}
1-2\delta^{r_2 \cubiii} \leq\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\in (1\pm\varepsilon)\sum_{i=1}^k \frac{1}{q}Z_i)\right)\leq\ppp\left( \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\in (1\pm4\varepsilon)k\right),
\end{gather*}
and again using that the $Z_i$'s and $N_i$'s are independent, we get that $\sum_{i=1}^k N_i^2Z_i/q\in (1\pm4\varepsilon)k$ holds with probability at least $(1-2\delta^{r_2 \cubiii})(1-4\delta^{\cubiii/3})\geq 1-6\delta^{\min(r_2,1/3)\cubiii}$.

\subsubsection*{Conclusion}
From the above, we see that in all cases, if we set $\cubiii$ as a sufficiently large constant, then with probability at least $1-\delta$, we have $\sum_{i=1}^k \frac{1}{q}N_i^2Z_i\in (1\pm 4\varepsilon)k$.  Since the analysis was done for an arbitrary $\varepsilon$ and $\delta$, it also hold for $\varepsilon'=\varepsilon/4$ and $\delta' = \delta/4$, thus we conclude that for $q=\max(\cubiiiii/m,(\cubii\varepsilon/4) \cdot \min\left (1,\ln (4k/\delta)/(m\ln(4/\varepsilon))\right ))$ we have that $ \sum_{i=1}^k \frac{1}{q}N_i^2Z_i\in (1\pm\varepsilon)k$ with probability $1-\delta/4$.
Since $\|Pu\|^2$ was equal in distribution to $\sum_{i=1}^k \frac{1}{q}N_i^2Z_i$, the same holds for $\|Pu\|^2$. 

In the above we had assumed that the vector $u$ had entries $u_i^2\leq 1/m$ and had unit length. By a similar argument to \cite{Ailon2009TheFJ} equation (4) page 308, we get that with probability at least $1-\delta/4$, it holds that $u_i^2=(HDx)_i^2\leq c_2'\ln (4d/\delta)/d$ for all $i=1\ldots,d$ simultaneously. Choosing $c_2\geq c_2'$ such that $1/m = 2 c_2 \ln(2n)/d$ is integer and constraining $\delta \leq 1/(nd)$, we get $u_i^2\leq 1/m$ as required.

Since $D$ is independent of $P$, we get that with probability at least $(1-\delta/4)(1-\delta/4) \geq 1-\delta/2$, we have $k^{-1}\|PHDx\|^2 \in (1 \pm \eps)$. 

For a set of $n$ vectors $X$, we may now choose $\delta = 1/(dn^3)$ and consider all normalized difference vectors $z/\|z\|$ with $z = x-y$ for $x,y \in X$. For any such $z$, define $u = HDz$. Since $HD$ is a unitary matrix, we have $\|u\| = \|z\|=1$. Moreover, by the above, we have $u_i^2 \leq c_2' \ln(4 n^3)/d$ for all $i$.

Now choosing $\delta=1/(4n^2)$ in the above, and $c_2\geq c_2'$ such that $u_i^2\leq 1/m=2c_2\ln (2n)/d$ is an integer, and noticing that $HD$ is a norm preserving mapping we have that the $u_x$'s has the properties as in the above. Now using a union bound over all the $n$ vectors in $X$ conditioned on the $u_x$'s satisfying the above we get that the event $\{\forall x\in X \text{ is such that } ||PHDx||^2\in (1\pm\varepsilon)k )\}$ holds with probability at least $(1-1/(4n))(1-1/(4n))\geq 1-1/(2n)$ and $q=\max(\cubiiiii/m,(\cubii \varepsilon)/(4)\min\left (1,\ln( 4n^2k)/(m\ln(4/\varepsilon))\right ))=O\left (\max(\frac{1}{m},\varepsilon\min\left (1,\ln (nk)/(m\ln\left(1/\eps \right))\right ))\right )$. 

We now claim that $q=O\left (\max(\ln n/d,\varepsilon\min\left (1,\ln^2 n/(d\ln\left(1/\eps \right))\right )\right )$ which would conclude the proof of \Cref{phdtheoremupper}. 
We first notice that if 
$\varepsilon\leq1/\ln n$ we have $$\frac{\varepsilon\ln (nk)}{m\ln\left(1/\eps \right)})=O\left (\frac{\ln (n\ln(n)/\varepsilon^2)}{d\ln\left(1/\eps \right)}\right )=O\left (\frac{ ((\ln n+\ln(\ln n)+2\ln\left(1/\eps \right)}{d\ln\left(1/\eps \right) }\right )=O(\ln (n)/d),$$ which is same order as the first term in the max. If $1/\ln n \leq\varepsilon\leq 1$ then $\ln(nk)=\Theta(\ln ((n\ln n)/(\varepsilon^2)))=\Theta(\ln n)$ so we conclude that $q=O\left (\max(\ln n/d,\varepsilon\min\left (1,\ln^2 n/(d\ln\left(1/\eps \right))\right )\right)$. which finish the proof of \cref{phdtheoremupper}


\end{proof}



\alert{Kasper: Remove below here}
\begin{proof}


The first two cases are simple: For $\delta$ less than a sufficiently small constant, we have $\alpha^2 qr = \ln(1/\delta)/36 < 3$. Moreover, if $\alpha > 1/2$, then $\sqrt{\ln(1/\delta)/(qr)}/6 > 1/2$, which implies $q \geq 9r/\ln(1/\delta)  = 9kd/(2^\ell \ln(1/\delta)) \geq 18 kd/\ln^2(1/\delta) \geq 18 k^2 /\ln^2(1/\delta) = \Omega(\eps^{-4})$. This is greater than $1$ for $\eps$ sufficiently small. 

Thus what remains is the case $\Pr[\sum_i b_i \geq qr + \sqrt{\ln(1/\delta)qr}] \geq \sqrt{\delta}$. Let us condition on $\sum_i b_i \geq qr + \sqrt{\ln(1/\delta)qr}$. Then by  with $x=0$ we get $\Pr[\sum_i b_i(N_i^2-1) \geq 0] \geq c_3$. This implies $\sum_i b_i N_i^2 \geq \sum_i b_i \geq qr + \sqrt{\ln(1/\delta)qr}$. But $\|Pu\|^2 = (2^\ell/(dq))(qr +  \sqrt{\ln(1/\delta)qr}) = k + \sqrt{\ln(1/\delta) 2^{2 \ell} r/(qd)} = k + \sqrt{\ln(1/\delta) 2^\ell k/(qd)}$. Thus with probability at least $c_3 \sqrt{\delta}$, we have $\|Pu\|^2 \geq k + \sqrt{\ln(1/\delta) 2^\ell k/(qd)}$. It follows that we must have 
\[
\sqrt{\ln(1/\delta) 2^\ell k/(qd)} \leq \eps k
\]
which implies $q \geq \eps^{-2} \ln(1/\delta) 2^\ell/d = \Omega(\ln(1/\delta)/d)$.


Since $\sum_{i=1}^\clbiiiii b_i$ is binomial distributed with success probability $q$ and $\clbiiiii d/2^\clbiiiiii$ trails its mean is $q\clbiiiii d/2^\clbiiiiii$. By Remark 1 in \cite{HAMZA199521}, we have with the definition of the $\text{median}$ of a binomial distribution as the smallest integer such that $P(X_{\text{Ber}(n,p)}\leq\text{median})>1/2$, that the median of a binomial distribution is close to its mean namely $|\text{median}-\text{mean}|\leq \min\{\ln2,\max\{p,1-p\}\}\leq 0.7$. By this fact we conclude that $\lfloor q\clbiiiii d/2^\clbiiiiii\rfloor$ is less than the median, since if $q\clbiiiii d/2^\clbiiiiii$ is an integer, the median, which is also an integer, must coincide with the mean since the gap between them is less than $0.7$, and if $q\clbiiiii d/2^\clbiiiiii$ is not an integer, then the median cannot be less than the integer part of $q\clbiiiii d/2^\clbiiiiii$, since the gap again is less than $0.7$. Hence concluding that $\lfloor q\clbiiiii d/2^\clbiiiiii\rfloor$ is a lower bound of the median.

Let now $A$ be the set of events where $\sum_{i=1}^k b_i$ is larger than its median and denote the median of $\sum_{i=1}^k b_i$ by $b_m$.  Let further $a_i$ denote the value of the $b_i$'s on the event $a\in A$. By the above we have that $q\clbiiiii d/2^\clbiiiiii\leq 0.7 +b_m$. Notice that we may assume that $q$ is so large that the median is strictly greater than 0, since otherwise we have at least probability $1/2$ of $\sum_{i=1}^k b_i=0$, hence mapping $u$ to the zero vector. By the above we then have that
\begin{gather}
\ppp\left[ \norm{Pu} >\clbiiiii +\sqrt{\frac{\clbiiiii2^{l-3}\ln\cphd}{dq\cphdi} }\right]\nonumber\\
=
\ppp\left[ \sum_{i=1}^\clbiiiii \left(\sum_{j=1}^{\frac{d}{2^\clbiiiiii}}  b_{i,j} N_{i,j}\right)^2
>\frac{\clbiiiii dq}{2^\clbiiiiii} +\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3} \cphdi}}\right]\nonumber\\
\geq
\sum_{a\in A}
\ppp\left[ \sum_{i=1}^\clbiiiii b_i N_i^2
>\frac{\clbiiiii dq}{2^\clbiiiiii} +\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3} \cphdi}} \Bigg| a \right]\ppp[a] \nonumber\\
\geq
\sum_{a\in A} \ppp\left[ \sum_{i=1}^\clbiiiii a_i N_i^2
>0.7+b_m +\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3} \cphdi}}\right]\ppp[a]\nonumber\\
=
\sum_{a\in A}\ppp\left[ \sum_{i=1}^\clbiiiii a_i N_i^2-b_m
> 0.7+\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3}\cphdi}}\right]\ppp[a]\nonumber\\
\geq
\sum_{a\in A}\ppp\left[ \sum_{i=1}^\clbiiiii a_i (N_i^2-1)
> 0.7+\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3} \cphdi}}\right]\ppp[a]\label{phdud1},
\end{gather}
where the last inequality uses that for $a\in A$ we have that $\sum_{i=1}^k a_i$ is greater than $b_m$, so setting $b_m=\sum_{i=1}^k a_i$ in the left hand side of the expression inside the probability decreases the probability and the inequality follows.

Now noticing that for each $a\in A$, $ \sum_{i=1}^\clbiiiii a_i (N_i^2-1)$ is a weighted sum of centred $\chi^2$-random variables we get by \Cref{reformulation restatement 1} that 
\begin{gather*}
\ppp\left[ \sum_{i=1}^\clbiiiii a_i (N_i^2-1)
> 0.7+\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3} \cphdi}}\right]\\
\geq
c_3\exp\left(-C_3\left(0.7+\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3} \cphdi}}\right)^2\Big/\sum_{i=1}^\clbiiiii a_i^2 \right)\\
\geq
c_3\exp\left(-C_3\left(2+\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+2} \cphdi}\right)\Big/\sum_{i=1}^\clbiiiii a_i \right)\\
\geq
c_3\exp\left(-C_3\left(2+\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+2} \cphdi}\right)\Big/\max\left\{1,\lfloor\frac{\clbiiiii dq}{2^{\clbiiiiii}}\rfloor\right\} \right)\\
\geq 
c_3\exp(-2C_3)\exp\left(-\frac{C_3 \ln \cphd}{2\cphdi} \right) \geq \sqrt{2\delta},
\end{gather*}
where we in the second inequality have used that the $a_i$'s are integers so less than or equal to their square and $(a+b)^2\leq 2a^2+2b^2$ for positive numbers $a,b$. The third inequality follows by that $\sum_{i=1}^k a_i$ is greater than or equal to the median which is lower bounded by the $\max\{1,\lfloor q\clbiiiii d/2^\clbiiiiii\rfloor\}$. In the second to last inequality we have used that $(\clbiiiii dq/2^\clbiiiiii)/\max\{1,\lfloor q\clbiiiii d/2^\clbiiiiii\rfloor\}$ is upper bound by $2$ and $2/\max\{1,\lfloor q\clbiiiii d/2^\clbiiiiii\rfloor\}$ is upper bounded by 2. Plugging the above into \cref{phdud1} we get that 

\begin{gather}
\ppp\left[ \norm{Pu} >k +\sqrt{\frac{k2^{l-3}\ln \cphd}{dq\cphdi} }\right]\nonumber\\
\geq
\sum_{a\in A}\ppp\left[ \sum_{i=1}^\clbiiiii a_i (N_i^2-1)
> 0.7+\sqrt{\frac{\clbiiiii dq\ln \cphd}{2^{\clbiiiiii+3} \cphdi}}\right ]\ppp[a]\label{phdud3}\\
\geq
\sum_{a\in A}\sqrt{2\delta}\ppp[a]
\geq \sqrt{\frac{\delta}{2}}\nonumber,
\end{gather}
and since we noticed (below \cref{phdud2}) that the probability of $Dx=x$ is at least $\sqrt{2\delta}$ it now follows by \cref{phdud3} that 
\begin{gather*}
\ppp\left[ \frac{1}{k}\norm{PHDx} >1 +\sqrt{\frac{2^{l-3}\ln \cphd}{kdq\cphdi} }\right] \nonumber\\
\ppp\left[ \norm{PHDx} >k +\sqrt{\frac{k2^{l-3}\ln \cphd}{dq\cphdi} }\right] \nonumber\\
\geq 
\ppp\left[ \norm{PHDx} >k +\sqrt{\frac{k2^{l-3}\ln \cphd}{dq\cphdi} }\Bigg| Dx=x \right] \ppp[ Dx=x]\\
=\ppp\left[ \norm{Pu} >k +\sqrt{\frac{k2^{l-3}\ln \cphd}{dq\cphdi} } \right ] \sqrt{2\delta}
\geq\delta.
\end{gather*}
Since we must have $\|Pu\|^2 \in (1 \pm \eps)k$ to preserve the norm of $x$, we conclude that:
\[
\varepsilon  \geq \sqrt{\frac{2^{l-3}\ln \cphd}{kdq\cphdi}}  \Rightarrow  q\geq \frac{2^{\clbiiiiii-3}\ln \cphd}{d\varepsilon^2k\cphdi}.
\]
Since we have by assumption that $\clbiiiii=\cphdii \ln(1/\delta)\varepsilon^{-2}$, by the definition of $\clbiiiiii$ have that $2^{\clbiiiiii}\geq \log_2(1/(\sqrt{2\delta}))/2\geq \ln(1/(\sqrt{2\delta}))/ (2\ln2)\geq\ln(1/\delta)/(8\ln2)$ for $\delta\leq 1/4$. If we also assume that $\delta\leq ({c_3^2/ (2e^{4C_3})})^{2}$, we have that $\ln \cphd\geq \ln (1/\delta)/4$ and conclude that 
\[
q \geq \frac{2^{\clbiiiiii-3}\ln \cphd}{d\varepsilon^2k\cphdi}
\geq \frac{\ln(1/\delta)\varepsilon^2 \ln(1/\delta)}{256\ln(2)d\varepsilon^2\cphdii\ln(1/\delta)C_3 }
\geq \frac{\ln(1/\delta)}{256\ln(2) C_3d \cphdii }=\frac{\clbxii \ln(1/\delta)}{d},
\]
with $\clbxii=1/(256\ln(2) C_3\cphdii)$. This concludes the first part of the proof of \Cref{phdtheorem2main} by assuming $\delta$ is less than a sufficiently small constant.
\end{proof}
\alert{Kasper: Remove up to this point}
